The Visualization JUDGE : Can Multimodal Foundation Models Guide Visualization Design Through Visual Perception?

Foundation models for vision and language are the basis of AI applications across numerous sectors of society. The success of these models stems from their ability to mimic human capabilities, namely visual perception in vision models, and analytical reasoning in large language models. As visual perception and analysis are fundamental to data visualization, in this position paper we ask: how can we harness foundation models to advance progress in visualization design? Specifically, how can multimodal foundation models (MFMs) guide visualization design through visual perception? We approach these questions by investigating the effectiveness of MFMs for perceiving visualization, and formalizing the overall visualization design and optimization space. Specifically, we think that MFMs can best be viewed as judges, equipped with the ability to criticize visualizations, and provide us with actions on how to improve a visualization. We provide a deeper characterization for text-to-image generative models, and multi-modal large language models, organized by what these models provide as output, and how to utilize the output for guiding design decisions. We hope that our perspective can inspire researchers in visualization on how to approach MFMs for visualization design.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/framework.tex <==
\section{Optimizing visualization design with vision-language models}

\subsection{Problem setup}

% notation for: (1) dataset, (2) visualization function, (3) parameters, (4) image output by visualization
Suppose that we are provided a dataset, denoted $\mathcal{D}$, that we wish to visualize.
We assume that the dataset can be represented as a list of $N$ data items $\mathcal{D} := ( \mathbf{x}_1, \mathbf{x}_2, \ldots , \mathbf{x}_N )$.
Each data item $\mathbf{x} \in \mathcal{D}$ is described by a collection of attributes $\mathcal{A} := \{ a_1, a_2, \ldots , a_M \}$, such that for $a \in \mathcal{A}$, $\mathbf{x}[a]$ gives the value of attribute $a$ for data item $\mathbf{x}$.
We further assume that a user has defined, a priori, a visualization method that will be used to visualize the dataset.
We represent this process of visualizing data as a function $\mathbf{V}$, one that accepts two inputs, (1) the dataset $\mathcal{D}$, and (2) a collection of visualization parameters $\mathbf{v} \in \mathbb{R}^D$, and outputs an image $\mathbf{I} = V(\mathcal{D}, \mathbf{v})$.

Designers often make choices on visualization parameters $\mathbf{v}$ when authoring a visualization.
The choices made on parameters are often informed by tasks that the resulting visualization should best support.
We may formalize these tasks as free-form text.

\subsection{Examples}

% concrete instantiations of the above formalism

Single-view visualizations.

Multiple-view visualizations.

Interactions?

Visualization algorithms (graph layouts, DR, ???).

Scientific visualization (color mapping, contouring, flow vis, volume rendering, ???).

\subsection{Vision-language models as differentiable visualization judges}

% purposing text-conditioned generative models as density models

% optimizing a visualization for a particular task <-> maximize the likelihood of a visualization output, subject to a user's task description

% what do we need?
    % 1. differentiable visualization, 

==> sections/suitability_LLM.tex <==
\subsection{Multimodal Large Language Model}

With the recent addition of visual modality, large language models have gained the ability to ``see''. Combined with their inherent knowledge and capability, the multimodal large language model (MLLM) significantly increased the potential applications compared to their language-only counterparts. One such application is on understanding and interpreting visualization. The promise of the proposed research direction hinged on the foundation models' capability to perceive and judge visualization, therefore, it is crucial to understand their abilities and key limitations.

Despite MLLM being a relatively new development, sizable research has been conducted on evaluating the fundamental vision capabilities of the MLLM model, from the early exploration \cite{yang2023dawn} that showcases their impressive abilities to more recent evaluations that reveal some of their key limitations \cite{fu2024blink} by focusing on harder tasks that require visual reasoning.
% Additionally, recent effort has been focusing on 
From basic chart and table visual question and answer benchmarks \cite{masry2022chartqa, mathew2022infographicvqa} to more recent developments in chart interpretation and task-based benchmarks \cite{xia2024chartx, wei2024mchartqa}. These evaluations and benchmarks provide valuable insight into general competence in various vision tasks and inspire further research that addresses identified shortcomings, such as localization/grounding \cite{cheng2024spatialrgpt}, and chart and table recognition \cite{}.

% yang2023dawn, yang2023dawn,masry2022chartqa, mathew2022infographicvqa, xia2024chartx, wei2024mchartqa

% \begin{itemize}
%     \item Existing evaluations on vision \cite{yang2023dawn, fu2024blink}
%     \item visualization-specific visual evaluation
%     \item shortcomings and challenges.
% \end{itemize}

In a related work by Zhimin et. al \cite{}, the author explored the state-of-the-art MLLM's capability for understanding visualization by leveraging the existing and well-curated visualization literacy test. The comparison results among the different models and against human experiments are illustrated in TABLE \ref{tab:VLAT_LLM_Task_data_table}.


ChatGPT give advice on visualization design \cite{kim2023good}

Explain visualization recommendation \cite{zhang2023adavis}

\begin{table*}[t]
\centering
\begin{tabular}{cccccccc}
 \hline
Task/LLM   & GPT4-o & Claude-opus & Gemini-1.5-pro & human \\  \hline
Retrieve Value(13)                                   & 0.461 & 0.338    & 0.361 & \textbf{0.621} \\
Find Extremum (12)                                & 0.683  & 0.491   & 0.675 & \textbf{0.782} \\ 
Determine Range (5)                               & 0.5  & 0.48     & \textbf{0.559 } & 0.492 \\
Find Correlations/Trends (5)                 & 0.82  & \textbf{0.820}      & 0.840  & 0.774 \\ 
Make Comparisons (12)                          & 0.575 & \textbf{0.75}   & 0.525  & 0.648 \\ 
Characterize Distribution (1)                 & 0.0      & 0.0     & 0.266 & \textbf{0.457 } \\ 
Find Anomalies (2)                                   & 0.35   & 0.2     & 0.2 & \textbf{0.485} \\ 
Find Clusters (2)                                        & \textbf{0.85}     & \textbf{0.85}     & 0.05 & 0.751 \\ 
identify the hierarchical structure (1)  & \textbf{1.0 }              & \textbf{1.0 }                & 0.9 & 0.879 \\ 
\hline
% All (53) maximum                                               &  0.660                  & 0.622                     & 0.566                &  \textbf{0.943} & -\\ 
% All (53) minimum                                                &  \textbf{0.547}                  & 0.452                     & 0.453                 & 0.339 &-\\ 
% All (53) mean                               & 0.586     & 0.545      & 0.518 & \textbf{0.667 } & 0.33 \\ 
%   \hline
\end{tabular}
\vspace{1mm}
\caption{The performance of MLLMs and humans on the visualization literacy task breakdown by visualization tasks.}
\label{tab:VLAT_LLM_Task_data_table}
\end{table*}

